Degeneracy-Locked Optical Parametric Oscillator

Optical parametric oscillators (OPOs) are widely utilized in photonics as classical and quantum light sources. Conventional OPOs produce co-propagating signal and idler waves that can be either degenerately or non-degenerately phase-matched. This configuration, however, makes it challenging to separate signal and idler waves and also renders their frequencies highly sensitive to external disturbances. Here, we demonstrate a degeneracy-locked OPO achieved through backward phase matching in a submicron periodically-poled thin-film lithium niobate microresonator. While the backward phase matching establishes frequency degeneracy of the signal and idler, the backscattering in the waveguide further ensures phase-locking between them. Their interplay permits the locking of the OPO's degeneracy over a broad parameter space, resulting in deterministic degenerate OPO initiation and robust operation against both pump detuning and temperature fluctuations. This work thus provides a new approach for synchronized operations in nonlinear photonics and extends the functionality of optical parametric oscillators. With its potential for large-scale integration, it provides a chip-based platform for advanced applications, such as squeezed light generation, coherent optical computing, and investigations of complex nonlinear phenomena.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
